Pipeline quantum processor architecture for silicon spin qubits

Noisy intermediate-scale quantum (NISQ) devices seek to achieve quantum advantage over classical systems without the use of full quantum error correction. We propose a NISQ processor architecture using a qubit `pipeline' in which all run-time control is applied globally, reducing the required number and complexity of control and interconnect resources. This is achieved by progressing qubit states through a layered physical array of structures which realise single and two-qubit gates. Such an approach lends itself to NISQ applications such as variational quantum eigensolvers which require numerous repetitions of the same calculation, or small variations thereof. In exchange for simplifying run-time control, a larger number of physical structures is required for shuttling the qubits as the circuit depth now corresponds to an array of physical structures. However, qubit states can be `pipelined' densely through the arrays for repeated runs to make more efficient use of physical resources. We describe how the qubit pipeline can be implemented in a silicon spin-qubit platform, to which it is well suited to due to the high qubit density and scalability. In this implementation, we describe the physical realisation of single and two qubit gates which represent a universal gate set that can achieve fidelities of $\mathcal{F} \geq 0.9999$, even under typical qubit frequency variations.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
